Binary Neutron Stars with Arbitrary Spins in Numerical Relativity

We present a code to construct initial data for binary neutron star systems in which the stars are rotating. Our code, based on a formalism developed by Tichy, allows for arbitrary rotation axes of the neutron stars and is able to achieve rotation rates near rotational breakup. We compute the neutron star angular momentum through quasi-local angular momentum integrals. When constructing irrotational binary neutron stars, we find a very small residual dimensionless spin of $\sim 2\times 10^{-4}$. Evolutions of rotating neutron star binaries show that the magnitude of the stars' angular momentum is conserved, and that the spin- and orbit-precession of the stars is well described by post-Newtonian approximation. We demonstrate that orbital eccentricity of the binary neutron stars can be controlled to $\sim 0.1\%$. The neutron stars show quasi-normal mode oscillations at an amplitude which increases with the rotation rate of the stars.

==> Makefile <==
#-----------------------------------------------------------------------
# $Id: Makefile 4 2007-12-14 06:18:35Z harald $
#-----------------------------------------------------------------------
AGR_FILES:=$(shell ls *.agr)
#AGR_FILES=
EPS_FIGURES2=$(shell ls *.eps)
EPS_FIGURES=$(AGR_FILES:%.agr=%.eps)
PDF_FIGURES=$(AGR_FILES:%.agr=%.pdf)


# typing 'make' will always 'latex paper' at least once.  If paper.tex
# has been modified, it will also execute the paper.dvi commands,
# resulting in the usual latex-bibtex-latex-latex combination to get
# all refereces right.

all: paper.pdf

nick: paper.pdf
	open /Applications/Adobe*Reader*.app paper.pdf

paper.dvi: $(EPS_FIGURES) $(EPS_FIGURES2) paper.tex
	latex paper
	bibtex paper
	latex paper
	latex paper


paper.ps: paper.dvi
	dvips -N0 -P pdf -t letter -o paper.ps paper.dvi

#paper.pdf: paper.ps
#	ps2pdf paper.ps

paper.pdf:  $(PDF_FIGURES) paper.tex
	pdflatex -draftmode -file-line-error paper
	bibtex paper
	pdflatex -draftmode -file-line-error paper
	pdflatex -file-line-error paper


# Automatically make postscript .eps files from .agr files
%.eps:%.agr
	xmgrace -hardcopy -hdevice EPS -printfile $@ $<

# Automatically make pdf files from .agr files
%.pdf:%.agr
	xmgrace -hardcopy -hdevice EPS -printfile epsfig.eps $<
	epstopdf --outfile=$@ epsfig.eps


# Automatically make postscript .eps files from .fig files
%.eps:%.fig
	fig2dev -L eps $< $@


# The || : is there to make sure that subsequent lines get executed even if
# some of the removes fail because the files to be removed do not exist.
clean:
	rm *.aux || :
	rm *.dvi || :
	rm *.log || :
	rm *.bbl || :
	rm *.blg || :
	rm $(FIGURES) || :
	rm $(PDFFIGURES) || :



PDFFIGURES=$(AGR_FILES:%.agr=%.pdf)
Mike: paper.tex $(PDFFIGURES) paper.bbl
	@(MakeFigLinks.sh)
	@(echo; echo "Running pdflatex"; echo )
	@(pdflatex paper.tex)
	@if grep -qi "Rerun" paper.log; \
	then \
		(echo; echo "Rerunning pdflatex"; echo); \
		(pdflatex paper.tex); \
		(echo; echo "Reran pdflatex once"; echo); \
	fi
	@if grep -qi "LaTeX Warning" paper.log; \
	then \
		(echo); \
		(echo "***************************************"); \
		(echo "* You may have an error in the LaTeX: *"); \
		(echo "***************************************"); \
		(echo ); \
		(grep -i "LaTeX Warning" paper.log); \
		(echo ); \
		(echo "***************************************"); \
	else \
		echo; \
	fi
paper.bbl : References/References.bib
	@(echo; echo "Running pdflatex and bibtex")
	@(pdflatex paper)
	@(bibtex paper)

